Utilization of Neighbor Information for Image Classification with Different Levels of Supervision

We propose to bridge the gap between semi-supervised and unsupervised image recognition with a flexible method that performs well for both generalized category discovery (GCD) and image clustering. Despite the overlap in motivation between these tasks, the methods themselves are restricted to a single task -- GCD methods are reliant on the labeled portion of the data, and deep image clustering methods have no built-in way to leverage the labels efficiently. We connect the two regimes with an innovative approach that Utilizes Neighbor Information for Classification (UNIC) both in the unsupervised (clustering) and semisupervised (GCD) setting. State-of-the-art clustering methods already rely heavily on nearest neighbors. We improve on their results substantially in two parts, first with a sampling and cleaning strategy where we identify accurate positive and negative neighbors, and secondly by finetuning the backbone with clustering losses computed by sampling both types of neighbors. We then adapt this pipeline to GCD by utilizing the labelled images as ground truth neighbors. Our method yields state-of-the-art results for both clustering (+3% ImageNet-100, Imagenet200) and GCD (+0.8% ImageNet-100, +5% CUB, +2% SCars, +4% Aircraft).

==> table-ablation-components.tex <==
\begin{table}[ht]
\caption{Ablation of the components (Imagenet-50 clustering)}
\label{tab:ablation_commponents}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}ccccc c@{}}
\toprule
 \multicolumn{4}{c}{Components in the pipeline} & \multicolumn{3}{c}{ImageNet-50 Clustering} \\
 \cmidrule(l){1-4}
 \cmidrule(l){5-7}
\multicolumn{1}{c}{Positives} & \multicolumn{1}{c}{Negatives} & \multicolumn{1}{c}{Entropy} & \multicolumn{1}{c}{Contrastive} & ACC  \\
\midrule
& & & & & \\
\checkmark & & & 17.64 & & \\
& \checkmark & & 89.48 & & \\
\checkmark & \checkmark & & \textbf{90.12} & & \\
\checkmark & & \checkmark & 14.12 & & \\
\checkmark & \checkmark & \checkmark & 88.24 & & \\
\bottomrule
\end{tabular}
}
\end{table}




==> table-ablation-gcd.tex <==
\begin{table}[ht]
\caption{Imagenet-100 Generalized Category Discovery Performance}
\label{tab:ablation_gcd}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}llllccc@{}}
\toprule
\multicolumn{2}{c}{\textbf{Positive Neighbors}} & \multicolumn{2}{c}{\textbf{Negative Neighbors}} & \multicolumn{3}{c}{\textbf{Accuracy}} \\ 
\cmidrule(l){1-2}
\cmidrule(l){3-4}
\cmidrule(l){5-7}
\textbf{Labelled} & \textbf{Unlabelled} & \textbf{Labelled} & \textbf{Unlabelled} & \textbf{All} & \textbf{Old} & \textbf{New} \\ 
\midrule
GT & Random & Random & Random & 82.22 & {\ul 92.36} & 77.13 \\
GT & Mined & Mined & Mined & \textbf{83.22} & 91.97 & \textbf{78.82} \\
GT & Mined & GT & Mined & {\ul 82.66} & \textbf{92.28} & {\ul 77.83} \\
\bottomrule
\end{tabular}
}
\end{table}




==> table-clustering-cifar.tex <==
\begin{table}[ht]
\caption{Image Clustering Results on Smaller Datasets}
\label{tab:clustering_cifar}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccc|ccc|ccc|ccc|}
          &           & \multicolumn{3}{c|}{CIFAR-10}         & \multicolumn{3}{c|}{CIFAR-20}             & \multicolumn{3}{c|}{CIFAR-100}            & \multicolumn{3}{c|}{XXX}               \\ \cline{3-14} 
Algorithm & Backbone  & ACC           & NMI       & New       & ACC               & NMI       & ARI       & ACC               & NMI       & ARI       & ACC               & NMI       & ARI       \\ \hline
kMeans    & Vit-B/16  & 83.60*        &           &           &                   &           &           & 56.99             &           &           &                   &           &           \\
SCAN~\cite{vangansbeke2020scan}      & Resnet-50 & 88.3          &           &           & 50.7              &           &           & 62.6+-0.94        &           &           & 80.9              &           &           \\
SPICE     & Resnet-50 & 92.6          &           &           & 53.8              &           &           &                   &           &           & 93.8              &           &           \\
TEMI~\cite{TEMI_BMVC2023}      & Vit-B/16  & 94.5          &           &           & 63.2              &           &           & 67.1+-1.30        &           &           & 98.5              &           &           \\ \hline
Ours      & Vit-B/16  & \textbf{89.0} & \textbf{} & \textbf{} & \textbf{Terrible} & \textbf{} & \textbf{} & \textbf{Terrible} & \textbf{} & \textbf{} & \textbf{Terrible} & \textbf{} & \textbf{}
\end{tabular}%
}
\end{table}


==> table-gcd-finegrained.tex <==
\begin{table}[t]
\caption{\textbf{Generalized Category Discovery Results on Fine Grained Datasets} reported for all, old, and new Classes.}
\label{tab:gcd_results_finegrained}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ll ccc ccc ccc@{}}
\toprule
& &\multicolumn{3}{c}{CUB-200} & \multicolumn{3}{c}{Aircrafts-100} & \multicolumn{3}{c}{SCars-196} \\ 
\cmidrule(l){3-5}
\cmidrule(l){6-8}
\cmidrule(l){9-11}
Algorithm & Backbone & All & Old & New & All & Old & New & All & Old & New \\ \midrule
kMeans  ~\cite{GCD_CVPR2022} &DINOv1 & 34.3 & 38.9 & 32.1 & 12.9 & 12.9 & 12.8 & 12.8 & 10.6 & 13.8\\
UNO+~\cite{fini2021unified} &DINOv1 & 35.1 & 49.0 & 28.1 & 28.3 & 53.7 & 14.7 & 35.5 & 70.5 & 18.6\\
ORCA~\cite{cao2021open} &DINOv1 & 36.3 & 43.8 & 32.6 & 31.6 & 32.0 & 31.4 & 31.9 & 42.2 & 26.9 \\
GCD~\cite{GCD_CVPR2022} &DINOv1 & 51.3 & 56.6 & 48.7 & 45.0 & 41.1 & 46.9 & 39.0 & 57.6 & 29.9 \\
DCCL~\cite{DCCL_CVPR2023} &DINOv1 & 63.5 & 60.8 & 64.9 & -- & -- & -- & 43.1 & 55.7 & 36.2 \\
Prompt CAL~\cite{Zhang_2023_CVPR} &DINOv1 & 62.9 & 64.4 & 62.1 & 52.2 & 52.2 & 52.3 & 50.2 & 70.1 & 40.6 \\ 
UNIC &DINOv1 &44.35 & 51.63 & 40.70 & 25.48 & 28.55 & 23.94 & --  & -- & --\\
SimGCD~\cite{Wen_2023_ICCV} &DINOv1 & 60.3 & 65.6 & 57.7 & 54.2 & 59.1 & 51.8 & 53.8 & 71.9 & 45.0  \\
\midrule
SPTnet~\cite{sptnet_iclr2024}&DINOv1+SimGCD  & \uline{65.8} & \uline{68.8} & \textbf{65.1}  & \uline{59.3} & \uline{61.8} & \uline{58.1} & \uline{59.0} & \uline{79.2} & \textbf{49.3} \\
UNIC (ours) &DINOv1+SimGCD & \textbf{69.42} & \textbf{83.39} & \uline{62.43} & \textbf{63.90} & \textbf{68.09} & \textbf{61.81} & \textbf{62.60}  & \textbf{90.71} & \uline{49.02} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> table-nei-cleaning.tex <==
\begin{table}[ht]
\caption{Variation of accuracy according to neighbor cleaning \mg{This should turn into Figure 5 and 6 later}}
\label{tab:nei_cleaning}
\resizebox{\textwidth}{!}{\%
\begin{tabular}{l|llllll|llllll|lllll}
 & \multicolumn{6}{c|}{10 Neighbor case}                                                                                                                                            & \multicolumn{6}{c|}{50 Neighbor case}                                                                                                                                            &  &  &  &  &  \\
 & \multicolumn{3}{c|}{Neighbors}                                                                    & \multicolumn{3}{c|}{Clustering}                                              & \multicolumn{3}{c|}{Neighbors}                                                                    & \multicolumn{3}{c|}{Clustering}                                              &  &  &  &  &  \\ \cline{2-13}
 & \multicolumn{1}{c}{Union Size} & \multicolumn{1}{c}{Remaining Nei} & \multicolumn{1}{c|}{Nei Acc} & \multicolumn{1}{c}{ACC} & \multicolumn{1}{c}{NMI} & \multicolumn{1}{c|}{ARI} & \multicolumn{1}{c}{Union Size} & \multicolumn{1}{c}{Remaining Nei} & \multicolumn{1}{c|}{Nei Acc} & \multicolumn{1}{c}{ACC} & \multicolumn{1}{c}{NMI} & \multicolumn{1}{c|}{ARI} &  &  &  &  &  \\ \cline{2-13}
 & 50                             & 56.08\%                            & \multicolumn{1}{l|}{97.93\%}  &                         &                         &                          & 100                            & 0.23\%                             & \multicolumn{1}{l|}{99.99\%}  &                         &                         &                          &  &  &  &  &  \\
 & 60                             & 81.45\%                            & \multicolumn{1}{l|}{97.08\%}  &                         &                         &                          & 200                            & 9.40\%                             & \multicolumn{1}{l|}{98.77\%}  &                         &                         &                          &  &  &  &  &  \\
 & 70                             & 94.41\%                            & \multicolumn{1}{l|}{95.71\%}  &                         &                         &                          & 300                            & 37.02\%                            & \multicolumn{1}{l|}{98.70\%}  &                         &                         &                          &  &  &  &  &  \\
 & 80                             & 98.93\%                            & \multicolumn{1}{l|}{94.43\%}  &                         &                         &                          & 400                            & 66.61\%                            & \multicolumn{1}{l|}{98.49\%}  &                         &                         &                          &  &  &  &  &  \\
 & 90                             & 99.99\%                            & \multicolumn{1}{l|}{93.90\%}  &                         &                         &                          & 500                            & 81.17\%                            & \multicolumn{1}{l|}{97.77\%}  &                         &                         &                          &  &  &  &  &  \\
 & 100                            & 100.00\%                           & \multicolumn{1}{l|}{93.89\%}  &                         &                         &                          & 1000                           & 96.69\%                            & \multicolumn{1}{l|}{93.53\%}  &                         &                         &                          &  &  &  &  &  \\
 &                                &                                   & \multicolumn{1}{l|}{}        &                         &                         &                          & 1500                           & 99.69\%                            & \multicolumn{1}{l|}{91.77\%}  &                         &                         &                          &  &  &  &  &  \\
 &                                &                                   & \multicolumn{1}{l|}{}        &                         &                         &                          & 2000                           & 100.00\%                           & \multicolumn{1}{l|}{91.55\%}  &                         &                         &                          &  &  &  &  &  \\
 &                                &                                   & \multicolumn{1}{l|}{}        &                         &                         &                          & 2500                           & 100.00\%                           & \multicolumn{1}{l|}{91.55\%}  &                         &                         &                          &  &  &  &  & 
\end{tabular}\%
}
\end{table}


==> table-scan-to-unic.tex <==
\begin{table}[h]
\caption{UNIC Ablation on Imagenet-50}
\label{tab:scan_to_unic}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{@{}ll ccc@{}}
\toprule
SCAN Loss & & - & - & - \\
SCAN Loss  & +VitB/16 & - & - & - \\
SCAN Loss  & +VitB/16 + Tune  - heads & - & - & - \\
SCAN Loss  & +VitB/16 + Tune  - heads & - & - & - \\
SCAN Loss  & +VitB/16 + Tune  - heads + cleaning & - & - & - \\
\midrule
UNIC & & - & - & - \\
\bottomrule

\end{tabular}
}
\end{table}

